Efficiency-Effectiveness Tradeoff of Probabilistic Structured Queries for Cross-Language Information Retrieval

Probabilistic Structured Queries (PSQ) is a cross-language information retrieval (CLIR) method that uses translation probabilities statistically derived from aligned corpora. PSQ is a strong baseline for efficient CLIR using sparse indexing. It is, therefore, useful as the first stage in a cascaded neural CLIR system whose second stage is more effective but too inefficient to be used on its own to search a large text collection. In this reproducibility study, we revisit PSQ by introducing an efficient Python implementation. Unconstrained use of all translation probabilities that can be estimated from aligned parallel text would in the limit assign a weight to every vocabulary term, precluding use of an inverted index to serve queries efficiently. Thus, PSQ's effectiveness and efficiency both depend on how translation probabilities are pruned. This paper presents experiments over a range of modern CLIR test collections to demonstrate that achieving Pareto optimal PSQ effectiveness-efficiency tradeoffs benefits from multi-criteria pruning, which has not been fully explored in prior work. Our Python PSQ implementation is available on GitHub(https://github.com/hltcoe/PSQ) and unpruned translation tables are available on Huggingface Models(https://huggingface.co/hltcoe/psq_translation_tables).

==> 8_limitation.tex <==
\section*{Limitations}

Our experiments do not carefully control the source and amount of parallel text
used to train neural translation models
and to build alignment matrices.
Since retrieval effectiveness depends on the quality of the translation models
(both neural MT models and the alignment matrix),
comparison across retrieval models would benefit from more controlled experimentation. 
There is also potentially a mismatch in vocabulary between the training data (including the parallel data and the query language uniform language model estimation data) and the documents being searched (especially for NeuCLIR collections which contain more recent documents), which could benefit from more experimentation as well. 
This problem also hinders a rigorous understanding of the cause of the trend differences across languages. 
We leave these controlled experiments to future work. 
